NEC: Speaker Selective Cancellation via Neural Enhanced Ultrasound Shadowing

In this paper, we propose NEC (Neural Enhanced Cancellation), a defense mechanism, which prevents unauthorized microphones from capturing a target speaker's voice. Compared with the existing scrambling-based audio cancellation approaches, NEC can selectively remove a target speaker's voice from a mixed speech without causing interference to others. Specifically, for a target speaker, we design a Deep Neural Network (DNN) model to extract high-level speaker-specific but utterance-independent vocal features from his/her reference audios. When the microphone is recording, the DNN generates a shadow sound to cancel the target voice in real-time. Moreover, we modulate the audible shadow sound onto an ultrasound frequency, making it inaudible for humans. By leveraging the non-linearity of the microphone circuit, the microphone can accurately decode the shadow sound for target voice cancellation. We implement and evaluate NEC comprehensively with 8 smartphone microphones in different settings. The results show that NEC effectively mutes the target speaker at a microphone without interfering with other users' normal conversations.

==> 2_0_threat_model.tex <==
\section{THREAT MODEL}\label{sec-threat-model}
The attacker's goal is to eavesdrop victim's voice in a public area. The voiceprint and the conversation content of the victim would be recorded intentionally. We assume that attackers neither have access to the victim's smart devices nor install any malicious recording applications on the victim's smart devices. Also, we assume the victim is in the public areas (e.g. cafe store, mall, canteen), and he/she has no awareness of being eavesdropped on.

\begin{itemize}[leftmargin=*]
    \item \textbf{Hidden Attack:} We assume that attacks can place/hide a recorder in advance as long as it's invisible to the victim. 
    \item \textbf{Attack Scenarios:} We assume that the victim is in the public areas, besides the victim, there are other people close to the victim that are using microphones for recording, making a phone call/video chat/online meeting.
    \item \textbf{No Awareness:} We assume the victim has no awareness of being eavesdropped on, he/she will speak at the normal volume.
\end{itemize}



==> keywords.tex <==
\begin{IEEEkeywords}
Noise Cancellation, Acoustics, Internet of Things, Edge Computing,
\end{IEEEkeywords}
